CrowdMoGen: Zero-Shot Text-Driven Collective Motion Generation

While recent advances in text-to-motion generation have shown promising results, they typically assume all individuals are grouped as a single unit. Scaling these methods to handle larger crowds and ensuring that individuals respond appropriately to specific events remains a significant challenge. This is primarily due to the complexities of scene planning, which involves organizing groups, planning their activities, and coordinating interactions, and controllable motion generation. In this paper, we present CrowdMoGen, the first zero-shot framework for collective motion generation, which effectively groups individuals and generates event-aligned motion sequences from text prompts. 1) Being limited by the available datasets for training an effective scene planning module in a supervised manner, we instead propose a crowd scene planner that leverages pre-trained large language models (LLMs) to organize individuals into distinct groups. While LLMs offer high-level guidance for group divisions, they lack the low-level understanding of human motion. To address this, we further propose integrating an SMPL-based joint prior to generate context-appropriate activities, which consists of both joint trajectories and textual descriptions. 2) Secondly, to incorporate the assigned activities into the generative network, we introduce a collective motion generator that integrates the activities into a transformer-based network in a joint-wise manner, maintaining the spatial constraints during the multi-step denoising process. Extensive experiments demonstrate that CrowdMoGen significantly outperforms previous approaches, delivering realistic, event-driven motion sequences that are spatially coherent. As the first framework of collective motion generation, CrowdMoGen has the potential to advance applications in urban simulation, crowd planning, and other large-scale interactive environments.

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> tables/kitml_quan.tex <==
\begin{table*}[h]
\centering
\caption{\textbf{Quantitative results on KIT-ML test set. }}
\label{tab:kitml_quan}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|ccccccc}
\toprule
\multirow{2}{*}{\centering\textbf{Method}} & \multirow{2}{*}{\centering\textbf{Joint}} & \multirow{2}{*}{\centering\textbf{FID $\downarrow$}} & \textbf{R-precision} & \multirow{2}{*}{\centering\textbf{Diversity $\rightarrow$}} & \multirow{2}{*}{\centering\textbf{Foot skating ratio} $\downarrow$} & \textbf{Traj. err.} & \textbf{Loc. err.} & \textbf{Avg. err.} \\ 
 &  &  & \textbf{(Top-3) $\uparrow$} &  &  & \textbf{(50 cm) $\downarrow$} & \textbf{(50 cm) $\downarrow$} & \textbf{(m) $\downarrow$} \\
\midrule
Real &  & 0.002 & 0.797 & 9.503 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
\midrule
PriorMDM~\cite{shafir2023human} & \multirow{4}{*}{\centering Pelvis} & 0.475 & 0.583 & 9.156 & 0.0897 & 0.3457 & 0.2132 & 0.4417 \\
GMD~\cite{karunratanakul2023guided} & & 0.576 & 0.665 & 9.206 & 0.109 & 0.0931 & 0.0321 & 0.1439  \\
OmniControl~\cite{xie2023omnicontrol} & & 0.218 & 0.687 & 9.422 & 0.0547 & 0.0387 & 0.0096 & 0.0338  \\
InterControl~\cite{wang2024intercontrol} & & 0.159 & 0.671 & 9.482 & 0.0729 & 0.0132 & 0.0004 & 0.0496 \\
\emph{Ours \textbf{CrowdMoGen}} & & 0.218 & 0.687 & 9.422 & 0.0547 & 0.0387 & 0.0096 & 0.0338 \\  
\midrule
OmniControl~\cite{xie2023omnicontrol} & \multirow{3}{*}{\centering Random One} & 0.310 & 0.693 & 9.502 & 0.0608 & 0.0617 & 0.0107 & 0.0404  \\
InterControl~\cite{wang2024intercontrol} & & 0.178 & 0.669 & 9.498 & 0.0968 & 0.0403 & 0.0031 & 0.0741 \\
\emph{Ours \textbf{CrowdMoGen}} & & 0.218 & 0.687 & 9.422 & 0.0547 & 0.0387 & 0.0096 & 0.0338 \\  
\midrule
InterControl~\cite{wang2024intercontrol} & \multirow{2}{*}{\centering Random Two} & 0.184 & 0.670 & 9.410 & 0.0948 & 0.0475 & 0.0030 & 0.0911 \\
\emph{Ours \textbf{CrowdMoGen}} & & 0.218 & 0.687 & 9.422 & 0.0547 & 0.0387 & 0.0096 & 0.0338 \\  
\midrule
InterControl~\cite{wang2024intercontrol} & \multirow{2}{*}{\centering Random Three} & 0.199 & 0.673 & 9.352 & 0.0930 & 0.0487 & 0.0026 & 0.0969 \\
\emph{Ours \textbf{CrowdMoGen}} & & 0.218 & 0.687 & 9.422 & 0.0547 & 0.0387 & 0.0096 & 0.0338 \\  
% Ours (on all) & Pelvis & 0.322 & 0.691 & 9.545 & 0.0571 & 0.0404 & 0.0085 & 0.0367 \\
% Ours (on all) & Left foot & 0.280 & 0.696 & 9.553 & 0.0692 & 0.0594 & 0.0094 & 0.0314 \\
% Ours (on all) & Right foot & 0.319 & 0.701 & 9.481 & 0.0668 & 0.0666 & 0.0120 & 0.0334 \\
% Ours (on all) & Head & 0.335 & 0.696 & 9.480 & 0.0556 & 0.0422 & 0.0079 & 0.0349 \\
% Ours (on all) & Left wrist & 0.304 & 0.680 & 9.436 & 0.0562 & 0.0801 & 0.0134 & 0.0529 \\
% Ours (on all) & Right wrist & 0.299 & 0.692 & 9.519 & 0.0601 & 0.0813 & 0.0127 & 0.0519 \\ 
% Ours (on all) & Average & 0.310 & 0.693 & 9.502 & 0.0608 & 0.0617 & 0.0107 & 0.0404 \\ 
\bottomrule
\end{tabular}%
}
\end{table*}
